Maximum n-times Coverage for Vaccine Design

We introduce the maximum $n$-times coverage problem that selects $k$ overlays to maximize the summed coverage of weighted elements, where each element must be covered at least $n$ times. We also define the min-cost $n$-times coverage problem where the objective is to select the minimum set of overlays such that the sum of the weights of elements that are covered at least $n$ times is at least $\tau$. Maximum $n$-times coverage is a generalization of the multi-set multi-cover problem, is NP-complete, and is not submodular. We introduce two new practical solutions for $n$-times coverage based on integer linear programming and sequential greedy optimization. We show that maximum $n$-times coverage is a natural way to frame peptide vaccine design, and find that it produces a pan-strain COVID-19 vaccine design that is superior to 29 other published designs in predicted population coverage and the expected number of peptides displayed by each individual's HLA molecules.

==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\I{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/abstract.tex <==





\begin{abstract}

We introduce the maximum $n$-times coverage problem that selects $k$ overlays to maximize the summed coverage of weighted elements, where each element must be covered at least $n$ times.   We also define the min-cost $n$-times coverage problem where the objective is to select the minimum set of overlays such that the sum of the weights of elements that are covered at least $n$ times is at least $\tau$.  Maximum $n$-times coverage is a generalization of the multi-set multi-cover problem, is NP-complete, and is not submodular.   We introduce two new practical solutions for $n$-times coverage based on integer linear programming and sequential greedy optimization. We show that maximum $n$-times coverage is a natural way to frame peptide vaccine design, and find that it produces a pan-strain COVID-19 vaccine design that is superior to 29 other published designs in predicted population coverage and the expected number of peptides displayed by each individual's HLA molecules.


\end{abstract} 
\vspace{-0.4in}

==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/conclusion.tex <==
\section{Conclusion}

We introduced the maximum $n$-times coverage problem, and showed that it is not submodular.   We presented both a novel ILP based method and a beam search algorithm for solving the problem, and used them to produce a peptide vaccine design for COVID-19.   We compared the resulting optimized peptide vaccine designs with 29 other published designs and found that the optimized designs provide substantially better population coverage for both MHC class I and class II presentation of viral peptides.  The use of $n$-times coverage as an objective increases vaccine redundancy and thus the probability that one of the presented peptides will be immunogenic and produce a T cell response.   We are presently testing our pan-strain COVID-19 vaccine in mouse challenge studies for protection against a COVID variant of concern.  Our pan-strain vaccine delivers MHC class I and class II $n$-times coverage optimized epitopes with a single mRNA-LNP construct.   Our methods can also be used to augment existing vaccine designs with peptides to improve their predicted population coverage by initializing the algorithm with peptides that are present in an existing design.
We provide an open-source implementation of our methods at \url{https://github.com/gifford-lab/optivax}.


==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/ilp.tex <==
\section{The \textsc{NTimes-ILP} solution for maximum $n$-times coverage}
\label{sec:ilp}

We first formulate the maximum-$n$ times coverage problem as an integer linear program (ILP). We associate a binary variable $a_i$ with each overlay $A_i$ such that $a_i=1$ if $A_i\in O^*$ and otherwise $a_i=0$. Thus the cardinality constraint can be written as $|O|=\sum_{i=1}^{m}a_i\leq k$, and the number of times an element $X_j$ is covered by $O$ is $C(X_j|O)=\sum_{i\in O}c_i(X_j)=\sum_{i=1}^m a_i c_i(X_j)$.
The main challenge is to encode the objective function $f_n(O) = \sum_{j=1}^{l}w(X_j)\mathbbm{1}_{\{\sum_{i=1}^m a_i c_i(X_j)\geq n\}}$ in a linear fashion. We replace the step function $\mathbbm{1}_{\{\sum_{i=1}^m a_i c_i(X_j)\geq n\}}$ with a variable $t_j$ such that for each element $X_j$:
\begin{equation}\label{eq:indicator}
    t_j = 1 \iff\sum_{i=1}^m a_i c_i(X_j) \geq n \quad \text{and}\quad t_j = 0 \iff \sum_{i=1}^m a_i c_i(X_j)< n
\end{equation}
We enforce the conditions in (\ref{eq:indicator}) with the Big M method~\citep{sherali_jarvis_bazaraa_2013}, where we include the following inequalities for each element $X_j\in \mathcal{X}$:
\begin{equation}
\label{eq-ilp}
    -M(1-t_j) \leq \sum_{i=1}^m a_i c_i(X_j) -n + \epsilon \leq Mt_j,
\end{equation}
We set $\epsilon \in (0,1)$ and choose $M$ to be a large number such as 10,000 which is larger than the term $\sum_{i=1}^m a_i c_i(X_j) -n + \epsilon$.  Here we prove that $t_j = 1 \iff \sum_{i=1}^m a_i c_i(X_j) \geq n$.  
\begin{proof}
When $t_j = 1$, inequality (\ref{eq-ilp}) becomes 
$0 \leq \sum_{i=1}^m a_i c_i(X_j) -n + \epsilon \leq M$.  
If $M$ is a large number, we can ignore the right inequality and rearrange to get 
$\sum_{i=1}^m a_i c_i(X_j) \geq n - \epsilon$.
Since $\sum_{i=1}^m a_i c_i(X_j)$ and $n$ are both integers and $\epsilon \in (0,1)$, we find
$\sum_{i=1}^m a_i c_i(X_j) \geq n.$
All these steps can be taken in the reverse order to prove that $\sum_{i=1}^m a_i c_i(X_j) \geq n \implies t_j = 1$, given that $t_j$ is a binary variable.
\end{proof}

We also prove that $t_j = 0 \iff \sum_{i=1}^m a_i c_i(X_j) < n$.  
\begin{proof}
We start by showing the forward direction.  If $t_j = 0$, then inequality (\ref{eq-ilp}) becomes
 $-M \leq \sum_{i=1}^m a_i c_i(X_j) -n + \epsilon \leq 0.$
 As $M$ is large, $-M$ is a large negative number, so we can ignore the left inequality.  Hence, 
 $\sum_{i=1}^m a_i c_i(X_j) \leq n - \epsilon < n.$
 In the reverse direction, if $\sum_{i=1}^m a_i c_i(X_j) < n$, because both the quantities $\sum_{i=1}^m a_i c_i(X_j)$ and $n$ are integers, for any $\epsilon \in (0,1)$, $\sum_{i=1}^m a_i c_i(X_j) \leq n-\epsilon$.  Rearranging this we get $\sum_{i=1}^m a_i c_i(X_j) - n + \epsilon \leq 0$, which forces $t_j$ as a binary variable to be equal to $0$ from inequality (\ref{eq-ilp}).
 \end{proof}

Therefore, the objective function to maximize becomes $f_n(O) = \sum_{j=1}^{l}w(X_j)\mathbbm{1}_{\{C(X_j|O)\geq n\}} = \sum_{j=1}^{l} t_j w(X_j)$, which is linear as a sum over $l$ terms of a binary variable multiplied by a constant.
 
The complete \textsc{NTimes-ILP} formulation of $n$-times coverage is:
\begin{outline}
    \1 Variables
        \2 $a_1, ..., a_m$ representing presence of each overlay $A_1, ..., A_m$ in final solution
        \2 $t_1, ..., t_l$ representing if each element $X_1, ..., X_l$ has been covered at least $n$ times
    \1 Constraints
        \2 $\sum_{i=1}^m a_i \leq k$ (the maximum total number of overlays allowed in the final subset)
        \2 $-M(1-t_j) \leq \sum_{i=1}^m a_i c_i(X_j) -n + \epsilon \leq Mt_j$ for each $j \in \{1, ..., l\}$
    \1 Objective to maximize
        \2 $f_n(O) = \sum_{j=1}^{l}w(X_j)\mathbbm{1}_{\{C(X_j|O)\geq n\}} = \sum_{j=1}^{l} t_j w(X_j)$
\end{outline}
If we want to enforce non-redundancy constraints such that pairs of overlays that violate certain distance criteria are not both chosen, we can include additional constraints $a_t + a_r \leq 1$ for every pair of overlays ($A_t$, $A_r$) that we don't want both to be included in the final subset.















==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

In the maximum $n$-times coverage problem, a set of overlays is selected to cover elements zero or more times, where each overlay is predetermined to cover one or more elements.  Each element is assigned a weight that reflects its importance.  The objective of the problem is to maximize the sum of the weights of elements that are covered at least $n$ times by at most $k$ overlays.   When the coverage of elements by overlays is determined by a machine learning method, the result summarizes machine learning results with a compact solution that is shaped by the element weights employed.

Our introduction of weighted elements and required $n$-times coverage creates a new class of problem without a known solution or complexity bound for approximate solutions. The closest problem to the maximum $n$-times coverage problem is the \emph{multi-set multi-cover problem} which does not assign weights to the elements and thus can be formulated as the Covering Integer Program (CIP) problem~\citep{srinivasan1999improved}.  Thus like CIP, maximum $n$-times coverage is NP-complete.   A $\log(n)$-time approximation algorithm for CIP can violate coverage constraints~\citep{dobson1982worst,kolliopoulos2003approximating,kolliopoulos2001tight}.  Deletion-robust submodular maximization protects against adversarial deletion~\citep{bogunovic2018robust,mirzasoleiman2017deletion} and robust submodular optimization protects against objective function uncertainty~\citep{iyer2019unified}, but neither guarantees that each element is covered $n$ times. 

In this work, we investigate properties of the maximum $n$-times coverage problem, provide a practical solution to the problem, and use the solution for machine learning based vaccine design.  We show that maximum $n$-times coverage is not submodular, and introduce \textsc{NTimes-ILP} and \textsc{MarginalGreedy}, efficient algorithms for solving the $n$-times coverage problem on both synthetic data and real vaccine design.   In our framing of vaccine design, an element is a specific collection of HLA alleles (a genotype), weights are the frequency of genotypes in the population, $n$ is the desired number of peptides displayed by each individual, and an overlay is a peptide that is predicted to be displayed by each genotype a specified number of times.   The solution of the maximum $n$-times coverage problem allows us to find a set of overlays that maximizes the sum of element weights (population coverage).   We show that framing vaccine design as maximum $n$-times coverage produces a solution that produces superior predicted population coverage when compared to 29 previous published vaccines for COVID-19 with less than 150 peptides.  











==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/optimization.tex <==
\section{The \textsc{MarginalGreedy} algorithm for maximum $n$-times coverage}
\label{sec:algorithm}

Although \textsc{NTimes-ILP} can produce near-optimal solutions on problems with reasonable size, it may become intractable for problems where hundreds of thousands of elements and/or overlays are involved, such as certain variants of the vaccine design problem. Thus, we seek a polynomial time algorithm that provides good solutions to the maximum $n$-times coverage problem.
A naive greedy solution is problematic when the $n$-times objective is directly approached.
This is a consequence of potential early bad overlay choices by a greedy approach that can cause it to fail later to find overlays with sufficient $n$-times coverage.
In addition, during greedy optimization available overlay choices may not provide differential marginal gain to avoid ties and random overlay selection. 
The \textsc{MarginalGreedy} algorithm is specifically designed to avoid early bad choices that will lead to failure by marginally approaching the $n$-times coverage objective.  
\textsc{MarginalGreedy} preserves marginal gains by employing look-ahead tie-breaking that assists in selecting overlays that benefit longer term objectives.
\begin{algorithm}[hb]
\caption{\textsc{MarginalGreedy} algorithm (for \textsc{Min-cost $n$-times Coverage})}
\label{algo:n_time}
\begin{algorithmic}
\State \textbf{Input:} Weights of the elements in $\mathcal{X}$: $w(X_1),w(X_2),\dots,w(X_l)$, ground set of overlays $\mathcal{A}$ where each overlay $j$ in $\mathcal{A}$ covers $X_i$ for $c_j(X_i)$ times, target minimum \# times being covered $n_{target}$, coverage cutoff for different $n$: $\tau_1,\tau_2,\dots,\tau_{n_{target}}$, beam size $b$
\State Initialize beam $B^0\leftarrow \{\emptyset\}$, $t=0$
\For{$n=1,\dots, n_{target}$}
    \State Using set function $f_n(S)=\sum_{i=1}^{l}w(X_i)\mathbbm{1}_{\{\sum_{j\in S}c_j(X_i)\geq n\}}$ as objective function.
    \Repeat
        \State $K^t\leftarrow\emptyset$ \Comment{$K^t$ is the set of candidate solutions}
        \For{$O \in B^t$} \Comment{Beam search}
            \For{$a\in\mathcal{A}\setminus O$}
                \State $K^t\leftarrow K^t\cup\{O\cup\{a\}\}$      \Comment{Add the candidate solution $\{O\cup\{a\}\}$ to $K^t$}
            \EndFor
        \EndFor
        \State $B^{t+1}\leftarrow$ \{Top $b$ candidate solutions in $K^t$ as scored by $f_n(S)$\}
        \State $t\leftarrow t+1$
        \State $m^t\leftarrow$ median score of candidate solutions in the beam $B^t$
    \Until{$m^t\geq\tau_n$ (in $n_{target}$-th cycle the termination condition is $\max_{S\in B^t}f_n(S)\geq\tau_{target}$)} 
    \State (for \textsc{Maximum $n$-times Coverage} with cardinality constraint $k$, there is additional
    \State termination condition $t>k$)
    \State $O^* = \argmax_{S\in B^t}f_{n_{target}}(S)$
\EndFor
\State \textbf{Output:} The final selected subset of overlays $O^*$
\end{algorithmic}
\end{algorithm}

\textsc{MarginalGreedy} optimizes $n$-times coverage with a sequence of greedy optimization cycles where the $n$-th cycle optimizes the coverage function $f_{n}(S)$.  
We establish coverage starting at $n=1$ and incrementally increase the $n$-times criteria to $n_{target}$. 
Thus early overlay selections are guided by less stringent
cycle-specific coverage objectives. A set of coverage cutoffs $\{\tau_1,\tau_2,\dots,\tau_{target}\}$ is used as the termination condition for each greedy optimization cycle, and when not specified, we assume $\tau_1=\tau_2=\dots=\tau_{target}$ by default. We use beam search to keep track of top $b$ candidate solutions at each iteration.   In general the larger the beam size, the closer the result is to the true optimal. However, there is a tradeoff between beam size and running time.  In our results we choose the largest beam size that maintains a practical running time as we describe below.

The full algorithm is given in Algorithm~\ref{algo:n_time}. A similar algorithm can be used to solve the \textsc{$n$-times Set Cover} problem in which $\tau_{target}=f_{n_{target}}(\mathcal{A})$. For the \textsc{Maximum $n$-times Coverage} problem with cardinality constraint $k$, the optimization terminates when $t>k$. When beam search is not used to reduce computation time ($b=1$), we have extended the algorithm to break ties during the $n$-times coverage iteration by looking ahead to $(n+1)$-times coverage.   We call this extension \textit{look ahead tie-breaking}. Another advantage of \textsc{MarginalGreedy} is that it is capable of guaranteeing high coverage for $n_t<n_{target}$ by controlling the cycle-specific coverage cutoffs $\tau_t$. This is desired in vaccine design where wider population coverage is also important and we want to make sure that almost 100\% of the population will be covered at least once.







==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/population.tex <==
\section{Vaccine population coverage maximization}
\label{sec:population}

Contemporary peptide vaccine design methods use machine learning scoring of peptide display for HLA alleles followed by the selection of peptides to maximize 1-times coverage.  These methods do not accurately model the frequency of HLA haplotypes in a population and thus can not accurately assess the population coverage provided by a vaccine.  \citet{malone2020artificial} uses haplotypes but does not explicitly model their frequencies.  For a selected set of peptides, the IEDB Population Coverage Tool~\citep{bui2006predicting} estimates peptide-MHC binding coverage and the distribution of peptides displayed for a given population but does not consider linkage disequilibrium between HLA loci.  

We frame vaccine design as maximum $n$-times coverage because ideally each vaccinated individual in a population will be ``covered'' by multiple immunogenic peptides.  While it might be assumed that an individual will be vaccinated if they display a single peptide, three independent lines of reasoning support the need for $n$-times coverage:

\begin{enumerate}
    \item When an individual displays multiple peptides their immune system activates and expands more than one set of T cell clonotypes that are poised to fight viral infection~\citep{sekine20,schultheis20,grifoni2020targets}.
    
    \item The peptides that are immunogenic vary from one individual to another, and thus having multiple peptides displayed increases the probability at least one will be strongly immunogenic~\citep{croft2019most}.
    
    \item If a virus evolves and changes its peptide composition, using multiple peptides reduces the chance of viral escape~\citep{wibmer2021}.
\end{enumerate}

Prior work has not considered formalizing these aspects of vaccine design with an $n$-times constraint and thus has produced solutions to the 1-times coverage task.  Existing solutions to 1-times coverage do not anticipate or solve the $n$-times coverage task. 
Both \citet{malone2020artificial} and \citet{toussaint2008mathematical} provide solutions to 1-times coverage, \citet{lundegaard2010popcover} does not provide specific population coverage guarantees, and \cite{oyarzun2015computer} reviews methods for 1-times coverage.  Discrete optimization has been used for other aspects of vaccine design that are unrelated to population coverage, such designing a single peptide sequence that covers a set of diverse but related set of input epitopes~\citep{theiler2018graph}, and designing spacers for string-of-beads peptide delivery~\citep{schubert2016designing}.






For a peptide to be effective in a vaccine it must be presented by an individual's Major Histocompatibility Complex (MHC) molecules and be immunogenic.  A displayed peptide is immunogenic when it activates T cells, which expand in number and mount a response against pathogens or tumor cells.  Memory T cells provide robust immunity against COVID-19, even in the absence of detectable antibodies~\citep{sekine20}.  The use of peptide vaccine components to activate T cells is in development for cancer~\citep{hu2018towards} and viral diseases including HIV~\citep{hivvaccine}, HPV~\citep{kenter2009vaccination} and malaria~\citep{li2014peptide,rosendahl2014t}.  

A challenge for the design of peptide vaccines is the diversity of human MHC alleles that each have specific preferences for the peptide sequences they will display.  The Human Leukocyte Antigen (HLA) loci, located within the MHC, encode the HLA class I and class II molecules.  We consider the three classical class I loci (HLA-A, HLA-B, and HLA-C) and three loci that encode class II molecules (HLA-DR, HLA-DQ, and HLA-DP). A single chromosome contains one allele at each locus.  We use \textit{haplotype} to represent a combination of HLA alleles in a single chromosome, denoted as $A_iB_jC_k$ for MHC class I or $DR_iDQ_jDP_k$ for MHC class II. Each haplotype has a frequency $G(i,j,k)$ in a given population where $\sum_{i=1}^{|\mathcal{A}|}\sum_{j=1}^{|\mathcal{B}|}\sum_{k=1}^{|\mathcal{C}|}G(i,j,k)=1$. Each individual inherits two haplotypes to form their diploid \textit{genotype} and may carry 3--6 different alleles per MHC class depending on the zygosity. The frequency of a diploid genotype is thus (MHC class I as an example):
\begin{equation}
\begin{split}
F^{i_1j_1k_1i_2j_2k_2} &= F(A_{i_1}B_{j_1}C_{k_1},A_{i_2}B_{j_2}C_{k_2})= G(i_1,j_1,k_1)G(i_2,j_2,k_2)
\end{split}
\end{equation}
We use observed frequencies of 2,138 MHC class I and 1,711 MHC class II haplotypes for our  population coverage optimization.  Each haplotype represents a specific combination of 230 different HLA-A, HLA-B, and HLA-C alleles (MHC class I) or 280 different HLA-DP, HLA-DQ, and HLA-DR alleles (MHC class II)~\citep{optivax2020}.  Our use of haplotypes models the linkage disequilibrium between HLA genes.
We separately select MHC class I and class II epitopes using $n$-times coverage and then combine them in a single vaccine delivery construct for an effective immune response.



We adopt an experimentally calibrated model of peptide-HLA immunogenicity to design vaccines using $n$-times coverage~\citep{optivaxaugmentation} (Appendix~\ref{sec:supp-filtering-details}).
We utilize the observed immunogenicity of peptides in convalescent COVID-19 patient peripheral blood mononuclear cell samples~\citep{snyder2020magnitude,klinger2015multiplex,nolan2020mira}, and use these data to select machine learning models to predict immunogenicity for peptides or HLA alleles that are not observed in the clinical data. %
We define a \textit{peptide-HLA hit} as a (peptide, HLA allele) pair where the peptide is predicted to be immunogenic and displayed by the HLA allele.
Once we have determined a candidate set of peptides that are predicted to be immunogenic, we then need to select a minimal subset of peptides such that each individual in $\tau_{target}$ of the population is predicted to have at least $n$ peptide-HLA hits.

We first introduce \textit{EvalVax-Robust}, an evaluation tool for estimating the population coverage of a proposed peptide vaccine set. \textit{EvalVax-Robust} evaluates the percentage of the population having at least $n$ peptide-HLA binding hits in each individual. For a given peptide $p$ and a class I HLA allele $X\in \mathcal{A}\cup\mathcal{B}\cup\mathcal{C}$, our machine learning model outputs a binary hit prediction $e_p(X)\in\{0,1\}$ indicating peptide-HLA immunogenicity.  For each diploid genotype we compute the total number of peptide-HLA hits as the sum of $e_p(X)$ over the unique HLA alleles in the genotype.
\begin{equation}
\begin{split}
c_p^{i_1j_1k_1i_2j_2k_2} &= c_p(A_{i_1}B_{j_1}C_{k_1},A_{i_2}B_{j_2}C_{k_2}) = \sum_{X \in \{A_{i_1},B_{j_1},C_{k_1}\}\cup\{A_{i_2},B_{j_2},C_{k_2}\}}e_p(X)
\end{split}
\end{equation}
The total number of peptide-HLA hits provided by a set of peptides $O$ is the sum of number of hits per peptide:
\begin{equation}
\begin{split}
C_O^{i_1j_1k_1i_2j_2k_2} &= C(A_{i_1}B_{j_1}C_{k_1},A_{i_2}B_{j_2}C_{k_2}|O) = \sum_{p\in O}c_p(A_{i_1}B_{j_1}C_{k_1},A_{i_2}B_{j_2}C_{k_2})
\end{split}
\end{equation}
We define the \textit{EvalVax-Robust} predicted population coverage with $\geq n$ peptide-HLA hits for a peptide vaccine set $P$ as:
\begin{equation}
\label{eq:coverage}
f_n(O) = \sum_{i_1=1}^{|\mathcal{A}|}\sum_{j_1=1}^{|\mathcal{B}|}\sum_{k_1=1}^{|\mathcal{C}|}\sum_{i_2=1}^{|\mathcal{A}|}\sum_{j_2=1}^{|\mathcal{B}|}\sum_{k_2=1}^{|\mathcal{C}|}F^{i_1j_1k_1i_2j_2k_2} \cdot \mathbbm{1} \{C_O^{i_1j_1k_1i_2j_2k_2} \geq n \}
\end{equation}
EvalVax-Robust population coverage optimization can be accomplished by a solution to the maximum $n$-times coverage problem, as we can rewrite equation (\ref{eq:coverage}) into equation (\ref{eq:objective}) by setting $\mathcal{X}$ to be the set of possible genotypes $i_1j_1k_1i_2j_2k_2$, and the weights $w(X_i)$ to be the genotype frequencies $F^{i_1j_1k_1i_2j_2k_2}$. The peptide candidate set is the set of possible overlays $\mathcal{A}$, where each peptide $p\in \mathcal{A}$ is an overlay which covers a genotype $c_p^{i_1j_1k_1i_2j_2k_2}$ times. We directly applied \textsc{MarginalGreedy} on EvalVax-Robust objective function with a beam size of 10 for MHC class I and 5 for MHC class II, but we further reduced peptide redundancy by eliminating unselected peptides that are within three (MHC class I) or five (MHC class II) edits on a sequence distance metric from the selected peptides at each iteration. The same non-redundancy constraints are added to \textsc{NTimes-ILP} as described in Section~\ref{sec:ilp}. As the number of unique genotypes is on the scale of millions (1M for MHC class I and 0.6M for MHC class II), for \textsc{NTimes-ILP} we used an alternative objective $f_n(O)_{hap}$ that computes $n$-times coverage at the haplotype level for better tractability. 
\begin{equation}
f_n(O)_{hap} = \sum_{i=1}^{|\mathcal{A}|}\sum_{j=1}^{|\mathcal{B}|}\sum_{k=1}^{|\mathcal{C}|}G(i,j,k) \cdot \mathbbm{1} \{C_O^{ijk} \geq n \}
\end{equation}


==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/problem.tex <==
\section{The Maximum $n$-times coverage problem}
\subsection{\textsc{Multi-set Multi-cover} problem}

In the standard \textsc{Set Cover} and \textsc{Maximum Coverage} problems, we are given a set $\mathcal{U}$ of $|\mathcal{U}|$ elements (also known as the universe) and a collection $\mathcal{S} = \{S_1,S_2,\dots,S_m\}$ of $m$ subsets of $\mathcal{U}$ such that $\bigcup_i S_i=\mathcal{U}$. The goal in the \textsc{Set Cover} problem is to select a minimal-cardinality set of subsets from $\mathcal{S}$ such that their union covers $\mathcal{U}$. The \textsc{Multi-set Multi-cover} (MSMC) problem is a generalization of the \textsc{Set Cover} problem, where multi-sets are sets in which an element can appear more than once.  The objective of the MSMC problem is to determine the minimum number of multisets (a multi-set can be chosen multiple times) such that each element $i$ is covered at least $b_i$ times. It can be formulated into Covering Integer Program (CIP) problem~\citep{srinivasan1999improved}:

\begin{definition}{(Covering Integer Program, CIP)}
\label{def:cip}
Given $A\in\mathbb{R}_+^{n\times m},b\in\mathbb{R}_+^n, w\in\mathbb{R}_+^m,d\in\mathbb{R}_+^m$, a CIP $P=(A,b,w,d)$ seeks to minimize $w^Tx$, subject to $Ax\geq b, x\in\mathbb{Z}_+^m$,and $x\leq d$.
\end{definition}
Here $A_{ij}$ represents the number of times $i$-th element appears in the $j$-th multi-set. The $w$ is set to be all 1 in MSMC. The constraints $x\leq b$ are called multiplicity constraints which limit the number of times a single multi-set can be reused, and they generally make covering problems much harder as natural linear programming (LP) relaxation can have an unbounded integrality gap~\citep{chuzhoy2006covering}. \citet{dobson1982worst} provides a combinatorial greedy $H(\max_j \sum_iA_{ij})$-approximation algorithm ($H(t)$ stands for $t$-th harmonic number) but multiplicity constraints can be dealt with effectively only in the (0,1) case, and thus this algorithm can be as bad as polynomial. \citet{kolliopoulos2001tight,kolliopoulos2003approximating} gave a tighter-bound solution that can obtain $O(\log n)$-approximation. 
\vspace{-0.1in}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm, clip=true]{figures/figure1.jpg}
    \vspace*{-1mm}
    \caption{Example of $n$-times coverage calculation.}
    \label{fig:illustrate}
\end{figure*}

\vspace{-0.2in}
\subsection{\textsc{Maximum $n$-times Coverage}}
We introduce the maximum $n$-times coverage problem, a variant of the MSMC problem that accounts for multiple coverage of each element while also assigning weights to different elements.  We are given a set $\mathcal{X}$ with $l$ elements $\{X_1,X_2,\dots,X_l\}$ each associated with a non-negative weight $w(X_i)$, and a set of $m$ overlays $\mathcal{A} = \{A_1,A_2,\dots,A_m\}$.  Each overlay $A_j$ covers each element $i$ in $\mathcal{X}$ an element specific number of times $c_j(X_i)$, which is similar to a multi-set.  When $c_j(X_i)=0$ the element $X_i$ is not covered by overlay $A_j$.
We use a very strict multiplicity constraint such that each overlay can be used only once. Given a subset of overlays $O \subseteq \mathcal{A}$, the total number of times an element $X_i$ is covered by $O$ is the sum of $c_j(X_i)$ for each overlay $j$ in $O$:
\begin{equation}
C(X_i|O)=\sum_{j\in O}c_j(X_i)
\end{equation}
We define the $n$-\textit{times coverage function} $f_n(O)$ as the sum of weights of elements in $\mathcal{X}$ that are covered at least $n$ times by $O$. Figure~\ref{fig:illustrate} shows an example computation of the $n$-\textit{times coverage function}.
\begin{equation}\label{eq:objective}
\begin{split}
    f_n(O) = \sum_{i=1}^{l}w(X_i)\mathbbm{1}_{\{C(X_i|O)\geq n\}} = \sum_{i=1}^{l}w(X_i)\mathbbm{1}_{\{\sum_{j\in O}c_j(X_i)\geq n\}}
\end{split}
\end{equation}
The objective of the \textsc{Maximum $n$-times Coverage} problem is to select a set of $k$ overlays $O \subseteq \mathcal{A}$ such that $f_n(O)$ is maximized. This can be formulated as the maximization of the monotone set function $f_n(O)$ under cardinality constraint $k$:
\begin{equation}
    O^*=\argmax_{O\subseteq \mathcal{A},|O|\leq k}f_n(O)
\end{equation}

We define \textsc{Min-cost $n$-times Coverage} as the minimum set of overlays such that the sum of the weights of elements covered at least $n$ times is $\geq \tau$.   We assume $\mathcal{A}$ provides sufficient $n$-times coverage for $f_n(\mathcal{A}) \geq \tau$.   We define the \textsc{$n$-times Set Cover} problem as the special case of \textsc{Min-cost $n$-times Coverage} where $\tau=\sum_iw(X_i)$.
\begin{equation}
    \text{\textsc{Min-cost $n$-times Coverage}}\quad\quad O^*=\argmin_{O}|O| \quad \text{s.t.} \quad f_n(O) \geq \tau
\end{equation}
\begin{equation}
    \text{\textsc{$n$-times Set Cover}} \quad\quad O^*=\argmin_{O}|O| \quad \text{s.t.} \quad f_n(O)=f_n(\mathcal{A})
\end{equation}

\begin{theorem}
The $n$-times coverage function $f_n(O)$ is not submodular.
\end{theorem}

The proof can be found in Appendix \ref{sec:submodular-proof}. Since the $n$-times coverage problem is not submodular, we cannot take advantage of the proven near-optimal performance of the greedy algorithm for the \textsc{Submodular Maximum Coverage} problem.  Thus we seek new solutions. 



==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/results.tex <==
\section{Results}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.82\linewidth]{figures/figure2-2.png}
    \vspace*{-2mm}
    \caption{The \textsc{MarginalGreedy} and \textsc{NTimes-ILP} algorithms outperform the greedy algorithm on both \textsc{LARGE} and \textsc{SMALL} toy examples. Superior performance is seen on both the \textsc{$n$-times Set Cover} where a smaller number of overlays is used by \textsc{MarginalGreedy} and \textsc{NTimes-ILP} to achieve 100\% coverage at different criteria of $n$, and on the \textsc{Maximum $n$-times Coverage} problems where \textsc{MarginalGreedy} and \textsc{NTimes-ILP} achieve higher coverage given same number of overlays.  Shaded regions indicate 95\% confidence intervals.}
    \label{fig:toy-results}
\end{figure*}

\subsection{Toy examples}
\label{sec:toy}
We empirically evaluate the \textsc{NTimes-ILP} and \textsc{MarginalGreedy} algorithms with two toy examples: a \textsc{LARGE} dataset where a set of 30 overlays are randomly generated to cover a set of 10 elements (with equal weights) 0, 1, or 2 times, and a \textsc{SMALL} dataset where a set of 10 overlays that were randomly generated to cover a set of 5 elements with equal weights 0, 1, or 2 times.
Figure~\ref{fig:toy-results} shows the efficiency of  the \textsc{NTimes-ILP}  and \textsc{MarginalGreedy} algorithms on both the \textsc{$n$-times Set Cover} and \textsc{Maximum $n$-times Coverage} problems for varying values of $n$.
We compare our algorithms to a greedy algorithm that directly optimizes $n$-times coverage and find the greedy algorithm degenerates to sub-optimal solutions for large values of $n$.   These sub-optimal solutions can be as bad as random.  We also compute the true optimal solution with exponential-time exhaustive search. 
We repeated problem generation and optimization with 6 different random seeds to provide confidence bounds and used beam size $b=1$ with look-ahead tie-breaking for \textsc{MarginalGreedy}. As shown in Figure~\ref{fig:toy-results},  \textsc{NTimes-ILP} achieves true optimal in all datasets and \textsc{MarginalGreedy} outperforms greedy on all tasks and datasets. We observed that \textsc{MarginalGreedy} has a significant advantage over greedy in tests with larger $n$ and in regions of higher coverage.
Appendix~\ref{sec:supp-more-toy} contains additional results for a more complex dataset with unequal element weights and sparser overlays, as well as a comparison to an additional local search baseline (hill climbing with restarts).



\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure3.png}
    \vspace*{-2mm}
    \caption{EvalVax population coverage evaluation of SARS-CoV-2 vaccines for (top) MHC class I and (bottom) MHC class II. (a) EvalVax-Robust population coverage with $n \geq 1$ peptide-HLA hits per individual, performances of 3 variants of OptiVax are shown by curves and baseline performance is shown by red crosses (labeled by name of first author). (b) EvalVax-Robust population coverage with $n \geq 5$ peptide-HLA hits. (c) EvalVax-Robust population coverage with $n \geq 8$ peptide-HLA hits. (d) Comparison of OptiVax and baselines on expected number of peptide-HLA hits. %
    }
    \label{fig:evalvax-results}
\end{figure*}


\subsection{COVID-19 vaccine design using maximum $n$-times coverage}
\label{sec:results-vaccine}

We used both the \textsc{NTimes-ILP} and \textsc{MarginalGreedy} algorithms to design peptide vaccines for COVID-19 and evaluated the population coverage with different number of HLA-peptide hits ($1\leq n \leq 8$) using EvalVax-Robust. %
For \textsc{MarginalGreedy} the time complexity of the algorithm is polynomial, $O(vbdp)$, where $v$ is the vaccine size, $b$ is the beam width, $d$ is the number of HLA diploid genotypes, and $p$ is the number of peptides.    For the COVID-19 vaccine problem, this is $O(10^{12})$, and our implementation typically takes 225 CPU hours (with parallelization it finishes in $<$1 hour) for vaccine design. By point of contrast, exhaustive search is ${p \choose v}d$, which is $O(10^{55})$.  

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure4-sm.png}
    \vspace*{-3mm}
    \caption{SARS-CoV-2 OptiVax selected peptide vaccine using \textsc{NTimes-ILP} on haplotypes for (A) MHC class I and (B) MHC class II.  (a) EvalVax-Robust population coverage at different per-individual number of peptide-HLA hit cutoffs for populations self-reporting as having White, Black, or Asian ancestry and average values. (b) Binding of vaccine peptides to each of the available alleles.}%
    \label{fig:optivax-results-ilp}
\end{figure*}

We compared our vaccine designs with 29 vaccine designs in the literature on the probability that a vaccine has at least $N$ peptide-HLA hits per individual in a population, and the expected number of per individual peptide-HLA hits in the population, which provides insight on how well a vaccine is displayed on average. %
Figure~\ref{fig:evalvax-results} shows the comparison between OptiVax (A) MHC class I and (B) class II vaccine designs at all vaccine sizes from 1--45 peptides (colored curves) and baseline vaccines (red crosses) from prior work.  We observe superior performance of OptiVax vaccine designs on all evaluation metrics at all vaccine sizes for both MHC class I and class II.  Most baselines achieve reasonable coverage at $n \geq 1$ peptide hits.  However, many fail to show a high probability of higher hit counts, indicating a lack of predicted redundancy if a single peptide is not displayed. Note that OptiVax-MarginalGreedy also outperforms all baselines on $n=1$ coverage and achieve 99.99\% (MHC class I) and 99.67\% (MHC class II) coverage for $n=1$, suggesting its capability to cover almost full population at least once while optimizing for higher peptide display diversity.
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/figure5-sm.png}
    \vspace*{-4mm}
    \caption{SARS-CoV-2 OptiVax selected peptide vaccine set using \textsc{MarginalGreedy}.}%
    \label{fig:optivax-results}
\end{figure*}
\paragraph{MHC class I results.}We selected an optimized set of peptides from all SARS-CoV-2 proteins using \textsc{NTimes-ILP} and \textsc{MarginalGreedy}. %
We use an MHC class I integrated model of peptide-HLA immunogenicity for our objective function.  After all filtering steps, we considered 1,100 candidate peptides.  With OptiVax-ILP, we design a vaccine with 19 peptides that achieves 99.999\% EvalVax-Robust coverage over populations self-reporting as having  Asian, Black, or White ancestry with at least one peptide-HLA hit per individual. This set of peptides also provides 98.52\% coverage with at least 5 peptide-HLA hits and 85.40\% coverage with at least 8 peptide-HLA hits (Figure~\ref{fig:optivax-results-ilp}A, Table~\ref{tab:baselines}).
With OptiVax-MarginalGreedy, we design a vaccine with 19 peptides that achieves 99.999\% EvalVax-Robust coverage over populations self-reporting as having  Asian, Black, or White ancestry with at least one peptide-HLA hit per individual. This set of peptides also provides 98.58\% coverage with at least 5 peptide-HLA hits and 87.97\% coverage with at least 8 peptide-HLA hits (Figure~\ref{fig:optivax-results}A, Table~\ref{tab:baselines}). The population level distribution of the number of peptide-HLA hits in White, Black, and Asian populations is shown in Figure~\ref{fig:optivax-results}A, where the expected number of peptide-HLA hits 11.355, 11.151 and 12.984, respectively.

\paragraph{MHC class II results.}
We use an MHC class II model of peptide-HLA immunogenicity for our objective function.  After all filtering steps, we considered 4,195 candidate peptides. With \textsc{NTimes-ILP}, we design a vaccine with 19 peptides that achieves 99.65\% EvalVax-Robust coverage with at least one peptide-HLA hit per individual. This set of peptides also provides 94.22\% coverage with at least 5 peptide-HLA hits and 83.76\% coverage with at least 8 peptide-HLA hits (Figure~\ref{fig:optivax-results-ilp}B, Table~\ref{tab:baselines}). With \textsc{MarginalGreedy}, we design a vaccine with 19 peptides that achieves 99.63\% EvalVax-Robust coverage with at least one peptide-HLA hit per individual. This set of peptides also provides 96.75\% coverage with at least 5 peptide-HLA hits and 87.35\% coverage with at least 8 peptide-HLA hits (Figure~\ref{fig:optivax-results-ilp}B, Table~\ref{tab:baselines}). The population level distribution of the number of peptide-HLA hits per individual in populations self-reporting as having Asian, Black, or White ancestry is shown in Figure~\ref{fig:optivax-results}B, where the expected peptide-HLA hits is 17.206, 16.085 and 11.210, respectively.

Table~\ref{tab:baselines} shows the evaluation of our OptiVax-Robust vaccine designs using the \textsc{MarginalGreedy} algorithm compared to 29 designs by others as baselines. We note that it is natural that our designs that were both optimized and evaluated with the same objective performed the best.  To provide a fair comparison, we also evaluated all designs with an immunogenicity model that does not incorporate clinical data and found that our designs also performed the best (Figure~\ref{fig:s1}).  The metric used in all cases is vaccine population coverage, which is a common metric~\citep{bui2006predicting}.  Thus, part of the contribution of the present work is emphasizing the value of combining machine learning predictions with combinatorial optimization for principled vaccine design.






==> Maximum n-times coverage -ICLR2022 (camera ready)_arXiv_fixtitle/sections/table_baselines.tex <==

\begin{table}[hbt]
    \centering
    \scriptsize
    \begin{tabular}{lR{0.8cm}R{1.1cm}R{1.1cm}R{1.1cm}R{0.9cm}R{0.9cm}R{0.9cm}R{0.9cm}}
    \toprule
   Peptide Set & Vaccine Size & EvalVax-Robust $p(n\geq1)$ & EvalVax-Robust $p(n\geq5)$ & EvalVax-Robust $p(n\geq8)$ & Exp. \# peptide-HLA hits / vaccine size & Exp. \# peptide-HLA hits (White) & Exp. \# peptide-HLA hits (Black) & Exp. \# peptide-HLA hits (Asian) \\
\midrule
\multicolumn{9}{l}{\textbf{MHC Class I Peptide Vaccine Evaluation}}\\
S-protein & $3795$ & $100.00$\% & $99.43$\% & $99.06$\% & $40.183$ & $38.212$ & $38.250$ & $44.086$ \\
S1-subunit & $2055$ & $100.00$\% & $99.05$\% & $97.37$\% & $20.788$ & $20.616$ & $20.397$ & $21.351$ \\
OptiVax-MarginalGreedy(Ours) & $19$ & $100.00$\% & $98.58$\% & $87.97$\% & $11.830$ & $11.355$ & $11.151$ & $12.984$ \\
OptiVax-ILP(Ours) & $19$ & $100.00$\% & $98.52$\% & $85.40$\% & $11.164$ & $10.883$ & $10.430$ & $12.180$ \\
\citet{srivastava2020structural} & $37$ & $99.90$\% & $80.06$\% & $44.74$\% & $7.163$ & $7.533$ & $7.018$ & $6.938$ \\
Random subset of binders & $19$ & $97.09$\% & $67.00$\% & $43.42$\% & $7.131$ & $7.368$ & $6.229$ & $7.796$ \\
\citet{fast2020potential} & $13$ & $89.60$\% & $57.38$\% & $30.55$\% & $5.558$ & $5.616$ & $4.386$ & $6.672$ \\
\citet{herst2020effective} & $52$ & $97.76$\% & $50.93$\% & $13.50$\% & $4.719$ & $5.207$ & $4.473$ & $4.477$ \\
\citet{lee2020silico} & $13$ & $75.78$\% & $42.18$\% & $20.60$\% & $4.113$ & $4.397$ & $3.384$ & $4.558$ \\
\citet{ahmed2020preliminary} & $16$ & $73.49$\% & $26.65$\% & $9.29$\% & $3.085$ & $3.051$ & $2.248$ & $3.957$ \\
\citet{herst2020effective} & $16$ & $96.70$\% & $13.97$\% & $0.07$\% & $2.931$ & $3.236$ & $2.988$ & $2.568$ \\
\citet{abdelmageed2020design} & $10$ & $79.09$\% & $7.05$\% & $0.11$\% & $2.000$ & $2.192$ & $1.777$ & $2.030$ \\
\citet{baruah2020immunoinformatics} & $5$ & $95.31$\% & $6.39$\% & $0.00$\% & $2.565$ & $3.128$ & $2.031$ & $2.537$ \\
\citet{gupta2020identification} & $7$ & $38.91$\% & $3.01$\% & $0.00$\% & $0.804$ & $0.747$ & $0.388$ & $1.278$ \\
\citet{singh2020designing} & $7$ & $67.80$\% & $2.84$\% & $0.00$\% & $1.499$ & $1.431$ & $1.305$ & $1.760$ \\
\citet{vashi2020understanding} & $51$ & $84.86$\% & $2.53$\% & $0.00$\% & $1.802$ & $1.976$ & $1.711$ & $1.720$ \\
\citet{poran2020sequence} & $10$ & $72.56$\% & $0.84$\% & $0.00$\% & $1.355$ & $0.997$ & $1.383$ & $1.686$ \\
\citet{khan2020design} & $3$ & $42.08$\% & $0.09$\% & $0.00$\% & $0.614$ & $0.702$ & $0.878$ & $0.263$ \\
\citet{akhand2020genome} & $31$ & $61.44$\% & $0.04$\% & $0.00$\% & $0.840$ & $1.062$ & $0.774$ & $0.682$ \\
\citet{bhattacharya2020development} & $13$ & $53.78$\% & $0.01$\% & $0.00$\% & $0.710$ & $0.977$ & $0.635$ & $0.518$ \\
\citet{saha2020silico} & $5$ & $39.30$\% & $0.00$\% & $0.00$\% & $0.423$ & $0.496$ & $0.291$ & $0.482$ \\
\citet{mitra2020multi} & $9$ & $32.13$\% & $0.00$\% & $0.00$\% & $0.355$ & $0.504$ & $0.251$ & $0.311$ \\
\midrule
\multicolumn{9}{l}{\textbf{MHC Class II Peptide Vaccine Evaluation}}\\
OptiVax-MarginalGreedy(Ours) & $19$ & $99.63$\% & $96.75$\% & $87.35$\% & $14.017$ & $16.989$ & $14.375$ & $10.686$ \\
S-protein & $16315$ & $99.28$\% & $96.53$\% & $96.04$\% & $395.096$ & $541.429$ & $416.406$ & $227.455$ \\
OptiVax-ILP(Ours) & $19$ & $99.65$\% & $94.22$\% & $83.76$\% & $13.540$ & $15.900$ & $14.762$ & $9.958$ \\
S1-subunit & $8905$ & $98.86$\% & $91.87$\% & $90.97$\% & $177.838$ & $265.183$ & $175.615$ & $92.717$ \\
\citet{ramaiah2020insights} & $134$ & $98.88$\% & $90.20$\% & $83.97$\% & $33.743$ & $45.044$ & $38.254$ & $17.932$ \\
Random subset of binders & $19$ & $93.70$\% & $59.13$\% & $32.47$\% & $6.033$ & $7.822$ & $6.527$ & $3.750$ \\
\citet{fast2020potential} & $13$ & $86.99$\% & $15.24$\% & $3.69$\% & $2.560$ & $3.650$ & $2.262$ & $1.769$ \\
\citet{banerjee2020energetics} & $9$ & $83.51$\% & $12.49$\% & $0.66$\% & $2.398$ & $3.162$ & $2.354$ & $1.679$ \\
\citet{akhand2020genome} & $31$ & $60.45$\% & $9.22$\% & $1.01$\% & $1.886$ & $2.531$ & $2.536$ & $0.591$ \\
\citet{singh2020designing} & $7$ & $56.29$\% & $0.96$\% & $0.00$\% & $0.981$ & $1.438$ & $1.113$ & $0.392$ \\
\citet{abdelmageed2020design} & $10$ & $28.40$\% & $0.96$\% & $0.00$\% & $0.479$ & $0.919$ & $0.274$ & $0.244$ \\
\citet{ulqamar2020designing} & $11$ & $72.75$\% & $0.27$\% & $0.00$\% & $1.278$ & $1.840$ & $1.464$ & $0.530$ \\
\citet{mitra2020multi} & $5$ & $47.92$\% & $0.04$\% & $0.00$\% & $0.657$ & $0.905$ & $0.579$ & $0.488$ \\
\citet{vashi2020understanding} & $20$ & $35.12$\% & $0.04$\% & $0.00$\% & $0.673$ & $0.959$ & $0.618$ & $0.442$ \\
\citet{poran2020sequence} & $10$ & $69.37$\% & $0.00$\% & $0.00$\% & $0.983$ & $1.469$ & $0.910$ & $0.569$ \\
\citet{ahmed2020preliminary} & $5$ & $54.96$\% & $0.00$\% & $0.00$\% & $0.654$ & $0.736$ & $0.717$ & $0.510$ \\
\citet{baruah2020immunoinformatics} & $3$ & $0.00$\% & $0.00$\% & $0.00$\% & $0.000$ & $0.000$ & $0.000$ & $0.000$ \\
\bottomrule
\end{tabular}
\caption{Comparison of existing baselines, S-protein peptides, and OptiVax-Robust peptide vaccine designs on various population coverage evaluation metrics. The rows are sorted by EvalVax-Robust $p(n \geq 1)$. Random subsets are generated 200 times. The binders used for generating random subsets are defined as peptides that are predicted to bind with $\leq$ 50 nM to more than 5 of the alleles.}
\label{tab:baselines}
\end{table}




